PromptRobust: Towards Evaluating the Robustness of Large Language Models on Adversarial Prompts

The increasing reliance on Large Language Models (LLMs) across academia and industry necessitates a comprehensive understanding of their robustness to prompts. In response to this vital need, we introduce PromptRobust, a robustness benchmark designed to measure LLMs' resilience to adversarial prompts. This study uses a plethora of adversarial textual attacks targeting prompts across multiple levels: character, word, sentence, and semantic. The adversarial prompts, crafted to mimic plausible user errors like typos or synonyms, aim to evaluate how slight deviations can affect LLM outcomes while maintaining semantic integrity. These prompts are then employed in diverse tasks including sentiment analysis, natural language inference, reading comprehension, machine translation, and math problem-solving. Our study generates 4,788 adversarial prompts, meticulously evaluated over 8 tasks and 13 datasets. Our findings demonstrate that contemporary LLMs are not robust to adversarial prompts. Furthermore, we present a comprehensive analysis to understand the mystery behind prompt robustness and its transferability. We then offer insightful robustness analysis and pragmatic recommendations for prompt composition, beneficial to both researchers and everyday users.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/tb-dataset-prompt-type-clean.tex <==
\begin{table}[t!]
\centering
\caption{Average performance and standard deviations of different prompts on different datasets.}
% \vspace{-.1in}
\label{tb-dataset-prompt-clean}
\resizebox{.48\textwidth}{!}{
\begin{tabular}{ccccc}
\toprule

Dataset  & ZS-task                      & ZS-role                      & FS-task                      & FS-role                      \\ \midrule
SST-2    & 76.85\scriptsize{$\pm$30.86} & 78.91\scriptsize{$\pm$25.91} & 76.0\scriptsize{$\pm$34.66}  & 72.97\scriptsize{$\pm$38.12} \\
CoLA     & 70.19\scriptsize{$\pm$18.68} & 71.83\scriptsize{$\pm$15.59} & 66.85\scriptsize{$\pm$25.54} & 67.5\scriptsize{$\pm$26.95}  \\
QQP      & 66.6\scriptsize{$\pm$32.25}  & 69.49\scriptsize{$\pm$27.75} & 72.24\scriptsize{$\pm$23.25} & 72.99\scriptsize{$\pm$22.44} \\
MRPC     & 67.99\scriptsize{$\pm$23.02} & 70.35\scriptsize{$\pm$20.52} & 75.64\scriptsize{$\pm$8.22}  & 75.68\scriptsize{$\pm$9.29}  \\
QNLI     & 69.92\scriptsize{$\pm$26.75} & 67.76\scriptsize{$\pm$28.49} & 73.15\scriptsize{$\pm$25.51} & 73.25\scriptsize{$\pm$24.79} \\
RTE      & 73.1\scriptsize{$\pm$22.81}  & 72.87\scriptsize{$\pm$24.33} & 69.96\scriptsize{$\pm$29.4}  & 71.89\scriptsize{$\pm$27.17} \\
WNLI     & 57.87\scriptsize{$\pm$16.39} & 57.82\scriptsize{$\pm$18.73} & 52.15\scriptsize{$\pm$26.67} & 55.85\scriptsize{$\pm$24.47} \\
MMLU     & 44.94\scriptsize{$\pm$14.58} & 45.33\scriptsize{$\pm$14.47} & 43.37\scriptsize{$\pm$21.11} & 43.28\scriptsize{$\pm$21.71} \\
SQuAD V2 & 80.13\scriptsize{$\pm$12.12} & 81.18\scriptsize{$\pm$10.31} & 82.78\scriptsize{$\pm$8.18}  & 83.17\scriptsize{$\pm$8.2}   \\
IWSLT    & 0.18\scriptsize{$\pm$0.03}   & 0.17\scriptsize{$\pm$0.04}   & 0.24\scriptsize{$\pm$0.01}   & 0.23\scriptsize{$\pm$0.01}   \\
UN Multi & 0.3\scriptsize{$\pm$0.03}    & 0.31\scriptsize{$\pm$0.03}   & 0.34\scriptsize{$\pm$0.02}   & 0.34\scriptsize{$\pm$0.02}   \\
Math     & 9.52\scriptsize{$\pm$4.74}   & 10.58\scriptsize{$\pm$3.64}  & 17.77\scriptsize{$\pm$2.52}  & 18.35\scriptsize{$\pm$2.7}  
\\
\bottomrule

\end{tabular}
}
% \vspace{-.2in}
\end{table}


==> tables/tb-dataset-promt.tex <==
\begin{table}[t!]
\centering
\caption{ADR on different prompts (ZS=zero-shot, FS=few-shot; ``-task'' and ``-role'' denote role-based or task-based prompts, respectively).}
\label{tb-dataset-prompt}
\resizebox{.5\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
Dataset             & ZS-task & FS-task & ZS-role & FS-role \\ \midrule
CoLA      & 0.30(0.23)     & 0.08(0.11)    & 0.24(0.23)     & 0.04(0.04)    \\
MNLI      & 0.10(0.20)     & 0.05(0.09)    & 0.05(0.11)     & 0.04(0.09)    \\
MRPC      & 0.13(0.19)     & 0.09(0.16)    & 0.18(0.27)     & 0.10(0.20)    \\
QNLI      & 0.17(0.22)     & 0.15(0.20)    & 0.26(0.34)     & 0.21(0.23)    \\
QQP       & 0.10(0.18)     & 0.05(0.12)    & 0.04(0.05)     & 0.05(0.08)    \\
RTE       & 0.06(0.11)     & 0.04(0.10)    & 0.05(0.09)     & 0.06(0.13)    \\
SST-2      & 0.05(0.16)     & 0.01(0.01)    & 0.10(0.18)     & 0.01(0.01)    \\
WNLI      & 0.10(0.13)     & 0.06(0.08)    & 0.08(0.10)     & 0.08(0.13)    \\
MMLU      & 0.12(0.20)     & 0.10(0.18)    & 0.05(0.06)     & 0.04(0.02)    \\
SQuAD\_V2 & 0.08(0.16)     & 0.06(0.14)    & 0.11(0.20)     & 0.03(0.09)    \\
IWSLT     & 0.14(0.16)     & 0.08(0.10)    & 0.22(0.17)     & 0.07(0.10)    \\
UN\_Multi & 0.16(0.15)     & 0.03(0.05)    & 0.17(0.13)     & 0.04(0.05)    \\
Math      & 0.34(0.25)     & 0.10(0.07)    & 0.34(0.27)     & 0.13(0.09)    \\ \midrule
Average      & 0.14(0.20)     & 0.07(0.12)    & 0.15(0.21)     & 0.07(0.13)  \\ \bottomrule 
\end{tabular}
}
\end{table}





==> tables/tb-falcon-10prompts.tex <==
\begin{table*}[htbp]
\caption{Results of 10 clean task-oriented prompts of Falcon-40B model on SST-2 dataset.}
\label{table: falcon 10 prompt}
\centering  
\begin{tabular}{c m{11.5cm}}
\toprule

\multicolumn{1}{c}{Accuracy}  & \multicolumn{1}{c}{Prompt} \\ \midrule
90.83    & {\scriptsize \prompt{Determine the overall sentiment of this sentence, categorizing it as 'positive' or 'negative':}}    \\ \midrule
87.61    & {\scriptsize \prompt{Please identify the emotional tone of this passage: 'positive' or 'negative'?}}                     \\ \midrule
83.60    & {\scriptsize \prompt{Given the context of this text, indicate if the emotion conveyed is 'positive' or 'negative':}}     \\ \midrule
77.98    & {\scriptsize \prompt{Read the provided excerpt and choose between 'positive' and 'negative' to describe its sentiment:}} \\ \midrule
62.73    & {\scriptsize \prompt{After examining the following expression, label its emotion as either 'positive' or 'negative':}}   \\ \midrule
59.40    & {\scriptsize \prompt{Evaluate the sentiment of the given text and classify it as 'positive' or 'negative':}}             \\ \midrule
11.47    & {\scriptsize \prompt{Analyze the tone of this statement and respond with either 'positive' or 'negative':}}              \\ \midrule
0.80     & {\scriptsize \prompt{Considering the given phrase, would you say it carries a 'positive' or 'negative' connotation?}}    \\ \midrule
0.69     & {\scriptsize \prompt{Assess the mood of the following quote and determine if it's 'positive' or 'negative':}}            \\ \midrule
0.00     & {\scriptsize \prompt{Review this statement and decide whether it has a 'positive' or 'negative' sentiment:}}  
\\

\bottomrule
\end{tabular}
%\end{center}
\end{table*}

==> tables/tb-falcon-atk-sst2.tex <==
\begin{table*}[htbp]
\caption{Results of different attacks on 6 prompts. P$i$ represents $i$-th prompt. The table entries in the A(B) format represent the model's accuracy on clean prompt (denote as A) and adversarial prompt (denote as B).}
\label{table: falcon atk sst2}
\centering  
\resizebox{\textwidth}{!}{
\begin{tabular}{c c cccccccc}
\toprule

\multicolumn{2}{c}{Attack}                 & TextBugger    & DeepWordBug  & TextFooler  & BertAttakc   & CheckList    & StressTest   & Semantic   \\
\midrule
\multirow{3}{*}{Task} & P1 & 90.83(4.70)   & 90.83(82.91) & 90.83(0.11) & 90.83(19.95) & 90.83(90.02) & 90.83(91.06) & 90.83(0.00) \\
                      & P2 & 87.61(2.29)   & 87.61(11.81) & 87.61(0.00) & 87.61(55.62) & 87.61(86.47) & 87.61(82.57) & 90.83(0.00) \\
                      & P3 & 83.60(25.80) & 83.60(1.03)  & 83.60(0.00) & 83.60(0.00)  & 83.60(83.83) & 83.60(77.52) & 90.83(0.00) \\
\midrule
\multirow{3}{*}{Role} & P4 & 83.83(2.52)   & 83.83(14.11) & 83.83(0.11) & 83.83(0.11)  & 83.83(83.72) & 83.83(82.22) & 90.83(0.11) \\
                      & P5 & 79.58(0.57)   & 79.59(1.95)  & 79.59(0.00) & 79.59(0.00)  & 79.59(74.77) & 79.59(75.57) & 90.83(0.46) \\
                      & P6 & 72.25(32.57)  & 72.25(43.23) & 72.25(0.00) & 72.25(0.00)  & 72.25(60.21) & 72.25(78.78) & 90.83(0.69)
\\
\midrule
\multicolumn{2}{c}{APDR} & 0.85\scriptsize{$\pm$0.17} &
0.69\scriptsize{$\pm$0.33} &
1.00\scriptsize{$\pm$0.00} &
0.86\scriptsize{$\pm$0.23} &
0.04\scriptsize{$\pm$0.06} &
0.02\scriptsize{$\pm$0.05} &
1.00\scriptsize{$\pm$0.00} &
\\
\bottomrule
\end{tabular}
}
%\end{center}
\end{table*}

==> tables/tb-human-eval.tex <==
\begin{table}[t!]
\centering
\caption{Acceptable rate of each attack on five volunteers.}
\label{tb-human-eval}
\resizebox{.48\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\toprule
    & BertAttack & DeepWordBug & TextBugger & TextFooler & Translation & Avg  \\
\midrule
V1  & 0.50        & 0.90         & 0.77       & 0.40        & 0.92        & 0.7  \\
V2  & 0.67       & 0.92        & 0.77       & 0.46       & 0.96        & 0.75 \\
V3  & 0.56       & 0.85        & 0.85       & 0.40        & 0.90         & 0.71 \\
V4  & 0.44       & 0.90         & 0.79       & 0.50        & 0.94        & 0.71 \\
V5  & 0.60        & 0.92        & 0.81       & 0.44       & 0.98        & 0.75 \\
\midrule
Avg & 0.55       & 0.90         & 0.80        & 0.44       & 0.94        & -    \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/tb-prompt-understanding.tex <==
\begin{table*}[t!]
\caption{Responses of LLMs that failed to understand prompts.}
\label{table: prompts understanding}
\centering  
\begin{tabular}{ m{2.7cm}  m{6cm} m{3.5cm}}
\toprule

LLMs and Datasets & Sample inputs & Response \\
% \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}

\midrule
LLaMa SST2 & \prompt{Evaluate the sentiment of the given text and classify it as 'positive' or 'negative': although laced with humor and a few fanciful touches , the film is a refreshingly serious look at young women .  Answer: } & analysis](https://en.wikipedia.org/wiki \\

\bottomrule
\end{tabular}
%\end{center}
\end{table*}
